Disentangling Uncertainty in Machine Translation Evaluation

Trainable evaluation metrics for machine translation (MT) exhibit strong correlation with human judgements, but they are often hard to interpret and might produce unreliable scores under noisy or out-of-domain data. Recent work has attempted to mitigate this with simple uncertainty quantification techniques (Monte Carlo dropout and deep ensembles), however these techniques (as we show) are limited in several ways -- for example, they are unable to distinguish between different kinds of uncertainty, and they are time and memory consuming. In this paper, we propose more powerful and efficient uncertainty predictors for MT evaluation, and we assess their ability to target different sources of aleatoric and epistemic uncertainty. To this end, we develop and compare training objectives for the COMET metric to enhance it with an uncertainty prediction output, including heteroscedastic regression, divergence minimization, and direct uncertainty prediction. Our experiments show improved results on uncertainty prediction for the WMT metrics task datasets, with a substantial reduction in computational costs. Moreover, they demonstrate the ability of these predictors to address specific uncertainty causes in MT evaluation, such as low quality references and out-of-domain data.

==> EMNLP 2022/combined_eval.tex <==
\begin{table}[t]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$  & NLL $\downarrow$ & PPS $\uparrow$\\  

  %0.086 & 0.017 & \underline{0.524} & 1.473 & 0.287 \\
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{WMT20 DA}}}  
& $\sigma^2$-fixed  & --    & 0.019  & 0.415  & 1.236 & 0.444 \\
& MCD   & 0.106 & 0.016  & \underline{0.377}  & 1.199 & 0.443 \\
  &  DE  & 0.134 & 0.019  & 0.366  & \underline{1.156} & \underline{0.460} \\
  & HTS & 0.177 & 0.015  & 0.450  & 1.201 & 0.444 \\
  & HTS+MCD & \underline{0.254} & \underline{0.013} & 0.528 & 1.167  & 0.429 \\ 
  & DUP  & 0.182 &	0.014 & 0.437 &	1.190 &	0.444\\[0.1cm]
  %0.112 & 0.015 & \underline{0.411} & 1.266 & 0.446 \\ % 
  \toprule
  \midrule

\multirow{6}{*}{\rotatebox{90}{\textsc{WMT21 MQM}}}  
& $\sigma^2$-fixed  & --  & 0.055  & 0.371  & 2.090 & 0.377 \\
& MCD & 0.179 & \underline{0.024} & 0.334 & 1.686 & 0.460 \\
& DE & 0.128 & 0.051 & \underline{0.236} & 2.631 & \underline{0.479} \\
& HTS  & 0.307  & 0.041  & 0.284  & 2.264  & 0.445  \\
& HTS+MCD  & \underline{0.311}  & 0.037  & 0.388  & \underline{1.614}  & 0.445  \\
& KL  & 0.296  & 0.046  & 0.273  & 2.595  & 0.443  \\
& DUP  & 0.285  & 0.039  & 0.634  & 1.778  & 0.377  \\ %   HTS + DEUP + Features (Trained on WMT20*0.7)
  %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{%\ricardo{Why is the PPS in the last column here and in the first column in Table 2} 
Results for segment-level DA and MQM predictions, averaged over all language pairs. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:combined}
\end{table}

% \underline{Underlined} numbers indicate the best result for each language pair and evaluation metric. Reported are the predictive Pearson score $r(\hat{\mu},q^*)$ (PPS), the uncertainty Pearson score $r(|q^*-\hat{\mu}|,\hat{\sigma})$ (UPS), the negative  log-likelihood (NLL), the expected calibration error (ECE), and the sharpness (Sha.)

% For calibration related indicators higher scores indicate lower performances. For correlation related indicators, higher scores indicate better performance. For each language pair the best values of each indicator are bold.

%% ORIGINAL copy
% \begin{table}[t]
% \small
% \centering
% \addtolength{\tabcolsep}{-0.5pt}
% \resizebox{7.7cm}{!}{
% \begin{tabular}{clccccc}
% \toprule
% &  & PPS $\uparrow$ & UPS $\uparrow$ & NLL $\downarrow$   & ECE $\downarrow$ & Sha. $\downarrow$ \\  
% \midrule
% \multirow{5}{*}{\rotatebox{90}{\textsc{En-Xx}}} 
% & MCD  & 0.601 & 0.128 & 0.616 & 0.032 & 0.673   \\
%   &  DE  & 0.631 & 0.134 & \underline{0.522} & 0.086 & 0.461 \\
%   & HTS  & 0.617 & 0.172 & 0.911 & 0.026 & 0.377 \\
%   & HTS+MCD & 0.609 &	\underline{0.323} &	0.994 &	0.017 &	0.516\\
%   & DUP  & \underline{0.633} & 0.145 & 1.021 & \underline{0.013} & \underline{0.293} \\%   HTS + DEUP + Features (Trained on WMT20*0.7)
%   %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  0.633 &	0.140 &	1.016 & 0.013	&	0.296   \\ 
%   \midrule
% \multirow{5}{*}{\rotatebox{90}{\textsc{Xx-En}}}  
% & MCD   & 0.286 & 0.019 & 1.033 & 0.073 & 1.432 \\
%   &  DE  & \underline{0.296} & 0.044 & \underline{0.943} & 0.086 & 1.131 \\
%   & HTS  & 0.278 & 0.079 & 1.441 & \underline{0.011} & 0.566 \\
%   & HTS+MCD & 0.276 &	\underline{0.176} &	1.323 &	\underline{0.011} &	0.600  \\
% %   & DEUP_{L1}  & 0.286 & 0.080 & 1.474 & 0.017 & 0.521 \\ %DEUP
% %   & DEUP_{L2} & 0.286 &	0.080 & 1.474 & 0.018 &	0.521  \\ %CZ to add
% %   & DEUP_{L3} &  &  &  &  & \\ % CZ to add: HTS + DEUP
%   & DUP  & 0.287 & 0.086 & 1.473 & 0.017 & \underline{0.524} \\%   HTS + DEUP + Features (Trained on WMT20*0.7)
%   %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} & 0.287	& 0.074 &	1.470 & 0.017	& 0.531  \\ 
%   \midrule
% \multirow{5}{*}{\rotatebox{90}{\textsc{Avg}}}  
% & MCD   & 0.435 & 0.071 & 0.816 & 0.053 & 1.083 \\
%   &  DE  & \underline{0.455} & 0.090 & \underline{0.728} & 0.086 & 0.813 \\
%   & HTS  & 0.435 & 0.119 & 1.189 & 0.020 & 0.466 \\
%   & HTS+MCD & 0.429 & \underline{0.254} &	1.167 &	\underline{0.013} &	0.528 \\ 
% %   & DEUP_{L1}  & 0.446 & 0.099 & 1.275 & 0.016 & 0.408 \\ 
% %   & DEUP_{L2} &0.446 & 0.105 &	1.279 &	0.017 &	0.427 \\ 
% %   & DEUP_{L3} &  &  &  &  & \\ % CZ to add: HTS + DEUP
%   & DUP  & 0.446 & 0.112 & 1.266 & 0.015 & \underline{0.411} \\ %   HTS + DEUP + Features (Trained on WMT20*0.7)
% %  & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} & 0.446  & 0.101 & 1.233 & 0.015 & 0.417  \\  
% \bottomrule
% \end{tabular}
% }
% \addtolength{\tabcolsep}{-0.5pt}
% \caption{Results for segment-level DA predictions. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
% \label{tab:da_seg_notqe}
% \end{table}

==> EMNLP 2022/sharpness_figs.tex <==
\begin{figure*}[hbt!]
\centering
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\textwidth]{images/ende-sharpness.pdf}
\subcaption{\textsc{En-De}}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\textwidth]{images/enru-sharpness.pdf}
\subcaption{\textsc{En-Ru}}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\textwidth]{images/zhen-sharpness.pdf}
\subcaption{\textsc{Zh-En}}
\end{subfigure}
\caption{Sharpness for in-domain \color{blue}(blue) \color{black} News WMT21 MQM data and out-of-domain \color{red}(red) \color{black} TEDTalks WMT21 MQM data. We show changes in sharpness values on each language pair separately, for the \textbf{DUP}, \textbf{HTS}, \textbf{MCD} and \textbf{DE} models finetuned on News WMT20 MQM data.  }
\label{fig:sharpness_ext}
\end{figure*}

==> EMNLP 2022/table_bleurt_full.tex <==
% \begin{table}[!h]
% \small
% \centering
% \addtolength{\tabcolsep}{-0.5pt}
% \resizebox{6cm}{!}{
% \begin{tabular}{clccccc}
% \toprule
% &  & UPS $\uparrow$ & ECE $\uparrow$ & Sha. $\downarrow$   & NLL $\downarrow$ & PPS $\downarrow$ \\  
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Cs}}}
%   & MCD & 0.226 & 0.235  & 1.031  & 2.000 & 0.399\\
%   & HTS & 0.291 & 0.071  & 3.727  & 1.848 & 0.386 \\
%   & HTS+MCD & 0.289 & 0.071  & 3.725  & 1.852 & 0.381 \\
%   & DUP & 0.410 & 0.079  & 5.029  & 1.986 & 0.400 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-De}}}
%  & MCD & 0.432 & 0.336  & 1.040  & 2.603 & 0.256\\
%  & HTS & 0.366 & 0.129  & 5.959  & 2.093 & 0.254 \\
%  & HTS+MCD & 0.358 & 0.128  & 5.846  & 2.083 & 0.248 \\
%  & DUP & 0.513 & 0.123  & 7.362  & 2.115 & 0.257 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Ja}}} & MCD & 0.326 & 0.358  & 1.041  & 2.592 & 0.275\\
%  & HTS & 0.278 & 0.126  & 5.105  & 2.003 & 0.293 \\
%  & HTS+MCD & 0.274 & 0.125  & 5.070  & 2.000 & 0.287 \\
%  & DUP & 0.420 & 0.124  & 7.295  & 2.122 & 0.277 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Pl}}}
%  & MCD & 0.217 & 0.247  & 1.032  & 2.105 & 0.347\\
%  & HTS & 0.262 & 0.070  & 3.779  & 1.870 & 0.341 \\
%  & HTS+MCD & 0.260 & 0.069  & 3.739  & 1.870 & 0.335 \\
%  & DUP & 0.362 & 0.076  & 5.092  & 1.992 & 0.349 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Ru}}} & MCD & 0.218 & 0.282  & 1.034  & 2.212 & 0.356\\
%  & HTS & 0.280 & 0.097  & 4.019  & 1.896 & 0.350 \\
%  & HTS+MCD & 0.275 & 0.096  & 4.010  & 1.895 & 0.345 \\
%  & DUP & 0.383 & 0.103  & 5.177  & 1.967 & 0.356 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Ta}}} & MCD & 0.131 & 0.218  & 1.029  & 2.047 & 0.240\\
%  & HTS & 0.320 & 0.062  & 3.499  & 1.826 & 0.248 \\
%  & HTS+MCD & 0.317 & 0.062  & 3.534  & 1.828 & 0.249 \\
%  & DUP & 0.279 & 0.060  & 4.501  & 1.966 & 0.240 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Zh}}} & MCD & 0.506 & 0.375  & 1.041  & 2.540 & 0.280\\
%  & HTS & 0.465 & 0.160  & 4.919  & 1.975 & 0.301 \\
%  & HTS+MCD & 0.449 & 0.160  & 4.920  & 1.974 & 0.297 \\
%  & DUP & 0.601 & 0.154  & 7.044  & 2.091 & 0.280 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Cs-En}}} & MCD & 0.303 & 0.202  & 1.030  & 1.924 & 0.059\\
%  & HTS & 0.291 & 0.073  & 2.775  & 1.735 & 0.052 \\
%  & HTS+MCD & 0.287 & 0.072  & 2.773  & 1.734 & 0.050 \\
%  & DUP & 0.360 & 0.068  & 3.781  & 1.838 & 0.061 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{De-En}}}  & MCD & 0.364 & 0.210  & 1.028  & 1.908 & 0.016\\
%  & HTS & 0.326 & 0.091  & 3.015  & 1.748 & -0.002 \\
%  & HTS+MCD & 0.323 & 0.091  & 3.000  & 1.746 & -0.003 \\
%  & DUP & 0.399 & 0.081  & 3.981  & 1.837 & 0.018 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Ja-En}}}  & MCD & 0.228 & 0.229  & 1.033  & 2.082 & 0.094\\
%  & HTS & 0.192 & 0.069  & 2.973  & 1.779 & 0.084 \\
%  & HTS+MCD & 0.184 & 0.068  & 2.948  & 1.777 & 0.082 \\
%  & DUP & 0.262 & 0.066  & 4.328  & 1.959 & 0.095 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Km-En}}}  & MCD & 0.084 & 0.145  & 1.029  & 1.827 & 0.205\\
%   & HTS & 0.100 & 0.026  & 2.168  & 1.642 & 0.209 \\
%  & HTS+MCD & 0.099 & 0.026  & 2.152  & 1.640 & 0.199 \\
%  & DUP & 0.149 & 0.021  & 3.222  & 1.856 & 0.208 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Pl-En}}}  & MCD & 0.313 & 0.213  & 1.031  & 2.002 & 0.053\\
%  & HTS & 0.253 & 0.069  & 2.842  & 1.766 & 0.057 \\
%  & HTS+MCD & 0.248 & 0.069  & 2.862  & 1.767 & 0.051 \\
%  & DUP & 0.358 & 0.067  & 3.922  & 1.919 & 0.053 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Ps-En}}}  & MCD & 0.176 & 0.151  & 1.029  & 1.861 & 0.088\\
%   & HTS & 0.165 & 0.033  & 2.058  & 1.647 & 0.075 \\
%   & HTS+MCD & 0.159 & 0.033  & 2.044  & 1.647 & 0.070 \\
%   & DUP & 0.218 & 0.028  & 3.267  & 1.859 & 0.090 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Ru-En}}}  & MCD & 0.261 & 0.228  & 1.030  & 1.986 & 0.076\\
%  & HTS & 0.219 & 0.087  & 3.135  & 1.786 & 0.068 \\
%  & HTS+MCD & 0.212 & 0.087  & 3.148  & 1.785 & 0.067 \\
%  & DUP & 0.319 & 0.081  & 4.021  & 1.897 & 0.076 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Ta-En}}}  & MCD & 0.238 & 0.121  & 1.020  & 1.688 & 0.106\\
%  & HTS & 0.245 & 0.046  & 1.704  & 1.561 & 0.098 \\
%  & HTS+MCD & 0.238 & 0.046  & 1.703  & 1.562 & 0.096 \\
%  & DUP & 0.273 & 0.034  & 2.959  & 1.767 & 0.108 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Zh-En}}}  & MCD & 0.309 & 0.231  & 1.033  & 2.075 & 0.079\\
%  & HTS & 0.278 & 0.078  & 2.984  & 1.790 & 0.071 \\
%  & HTS+MCD & 0.270 & 0.078  & 2.984  & 1.790 & 0.068 \\
%  & DUP & 0.353 & 0.075  & 4.252  & 1.932 & 0.080 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Xx}}}  & MCD & 0.302 & 0.295  & 1.035  & 2.291 & 0.316\\
%   & HTS & 0.328 & 0.104  & 4.383  & 1.925 & 0.319 \\
%  & HTS+MCD & 0.322 & 0.103  & 4.364  & 1.924 & 0.314 \\
%  & DUP & 0.435 & 0.105  & 5.917  & 2.033 & 0.317 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Xx-En}}}  & MCD & 0.274 & 0.204  & 1.030  & 1.965 & 0.079\\
%  & HTS & 0.246 & 0.069  & 2.755  & 1.739 & 0.071 \\
%  & HTS+MCD & 0.240 & 0.069  & 2.753  & 1.739 & 0.068 \\
%  & DUP & 0.320 & 0.064  & 3.892  & 1.888 & 0.080 \\
%  \midrule
%  \multirow{4}{*}{\rotatebox{90}{\textsc{AVG}}}  & MCD & 0.287 & 0.247  & 1.032  & 2.120 & 0.191\\
%  & HTS & 0.285 & 0.086  & 3.527  & 1.827 & 0.189 \\
%  & HTS+MCD & 0.279 & 0.085  & 3.517  & 1.827 & 0.185 \\
%  & DUP & 0.374 & 0.083  & 4.853  & 1.957 & 0.192 \\
% \bottomrule
% \end{tabular}
% }
% \addtolength{\tabcolsep}{-0.5pt}
% \caption{Results for segment-level DA prediction for BLEURT. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
% \label{tab:da_bleurt}
% \end{table}



% AVERAGE
\begin{table}[ht]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$   & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Xx}}}  
  & $\sigma^2$-fixed & -- &  0.107  & 4.698  & 1.984 & 0.317 \\
  & MCD & 0.302 & 0.295  & \underline{1.035}  & 2.291 & 0.316 \\
  & DE & 0.204 & 0.205  & 1.886  & 2.034 & \underline{0.337} \\
  & HTS & 0.328 & 0.104  & 4.383  & 1.925 & 0.319 \\
  & HTS+MCD & 0.322 & \underline{0.103}  & 4.364  & \underline{1.924} & 0.314 \\
  & DUP & \underline{0.435} & 0.105  & 5.917  & 2.033 & 0.317 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Xx-En}}}  
  & $\sigma^2$-fixed & -- & 0.067  & 3.200  & 1.831 & 0.080  \\
  & MCD & 0.274 & 0.204  & \underline{1.030}  & 1.965 & 0.079 \\
  & DE & 0.032 & 0.107 & 1.392 & 1.845 & \underline{0.111} \\
  & HTS & 0.246 & 0.069  & 2.755  & \underline{1.739} & 0.071 \\
  & HTS+MCD & 0.240 & 0.069  & 2.753  & \underline{1.739} & 0.068 \\
  & DUP & \underline{0.320} & \underline{0.064}  & 3.892  & 1.888 & 0.080 \\
 \midrule
 \multirow{6}{*}{\rotatebox{90}{\textsc{AVG}}}  
  & $\sigma^2$-fixed & -- &  0.086  & 3.910  & 1.903 & 0.192 \\
  & MCD & 0.287 & 0.247  & \underline{1.032}  & 2.120 & 0.191 \\
  & DE & 0.172 & 0.150 & 1.608  & 1.926 & \underline{0.210} \\
  & HTS & 0.285 & 0.086  & 3.527  & \underline{1.827} & 0.189 \\
  & HTS+MCD & 0.279 & 0.085  & 3.517  & \underline{1.827} & 0.185 \\
  & DUP & \underline{0.374} & \underline{0.083}  & 4.853  & 1.957 & 0.192 \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level DA predictions by BLEURT  [\textbf{Average across language pairs}]. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_bleurt_all}
\end{table}

% En-Xx pairs
\begin{table}[ht]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$   & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Cs}}}
  & $\sigma^2$-fixed & -- & 0.083  & 3.462  & 1.860 & 0.400 \\
  & MCD & 0.226 & 0.235  & \underline{1.031}  & 2.000 & 0.399\\
  & DE & 0.326 & 0.161  & 1.656  & \underline{1.846} & \underline{0.446} \\
  & HTS & 0.291 & \underline{0.071}  & 3.727  & 1.848 & 0.386 \\
  & HTS+MCD & 0.289 & \underline{0.071}  & 3.725  & 1.852 & 0.381 \\
  & DUP & \underline{0.410} & 0.079  & 5.029  & 1.986 & 0.400 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-De}}}
  & $\sigma^2$-fixed & -- & \underline{0.112}  & 5.779  & 2.099 & 0.257\\
  & MCD & 0.432 & {0.336}  & \underline{1.040}  & 2.603 & 0.256\\
  & DE & 0.198 & 0.217  & 2.508  & 2.207 & \underline{0.267} \\
  & HTS & 0.366 & 0.129  & 5.959  & 2.093 & 0.254 \\
  & HTS+MCD & 0.358 & 0.128  & 5.846  & \underline{2.083} & 0.248 \\
  & DUP & \underline{0.513} & 0.123  & 7.362  & 2.115 & 0.257 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ja}}} 
  & $\sigma^2$-fixed & -- & 0.134  & 6.040  & 2.105 & 0.277 \\
  & MCD & 0.326 & 0.358  & \underline{1.041}  & 2.592 & 0.275\\
  & DE & 0.121 & 0.258  & 1.937  & 2.185 & 0.289 \\
  & HTS & 0.278 & 0.126  & 5.105  & 2.003 & \underline{0.293} \\
  & HTS+MCD & 0.274 & 0.125  & 5.070  & \underline{2.000} & 0.287 \\
  & DUP & \underline{0.420} & \underline{0.124}  & 7.295  & 2.122 & 0.277 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Pl}}}
  & $\sigma^2$-fixed & -- & 0.081  & 3.739  & 1.904 & 0.349\\
  & MCD & 0.217 & 0.247  & \underline{1.032}  & 2.105 & 0.347\\
  & DE & 0.247 & 0.154  & 1.728  & 1.876 & \underline{0.374} \\
  & HTS & 0.262 & 0.070  & 3.779  & \underline{1.870} & 0.341 \\
  & HTS+MCD & 0.260 & \underline{0.069}  & 3.739  & \underline{1.870} & 0.335 \\
  & DUP & \underline{0.362} & 0.076  & 5.092  & 1.992 & 0.349 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ru}}} 
  & $\sigma^2$-fixed & -- & 0.100  & 4.321  & 1.959 & 0.356 \\
  & MCD & 0.218 & 0.282  & \underline{1.034}  & 2.212 & 0.356 \\
  & DE & 0.158 & 0.184  & 1.838  & 1.951 & \underline{0.361} \\
  & HTS & 0.280 & 0.097  & 4.019  & 1.896 & 0.350 \\
  & HTS+MCD & 0.275 & \underline{0.096}  & 4.010  & \underline{1.895} & 0.345 \\
  & DUP & \underline{0.383} & 0.103  & 5.177  & 1.967 & 0.356 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ta}}} 
  & $\sigma^2$-fixed & -- & 0.065  & 3.530  & 1.877 & 0.240 \\
  & MCD & 0.131 & 0.218 & \underline{1.029} & 2.047 & 0.240 \\
  & DE & 0.162 & 0.135  & 1.822  & 1.864 & \underline{0.278} \\
  & HTS & \underline{0.320} & 0.062  & 3.499  & \underline{1.826} & 0.248 \\
  & HTS+MCD & 0.317 & 0.062  & 3.534  & 1.828 & 0.249 \\
  & DUP & 0.279 & \underline{0.060}  & 4.501  & 1.966 & 0.240 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Zh}}} 
  & $\sigma^2$-fixed & -- & \underline{0.154}  & 6.063  & 2.097 & 0.280 \\
  & MCD & 0.506 & 0.375 & \underline{1.041} & 2.540 & 0.280 \\
  & DE & 0.171 & 0.297  & 1.940  & 2.297 & 0.282 \\
  & HTS & 0.465 & 0.160  & 4.919  & 1.975 & \underline{0.301} \\
  & HTS+MCD & 0.449 & 0.160  & 4.920  & \underline{1.974} & 0.297 \\
  & DUP & \underline{0.601} & \underline{0.154}  & 7.044  & 2.091 & 0.280 \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level DA predictions by BLEURT for En-Xx LPs. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_bleurt_enxx}
\end{table}



% Xx-En pairs
\begin{table}[ht]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$   & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Cs-En}}} 
  & $\sigma^2$-fixed & -- & \underline{0.068}  & 3.085  & 1.816 & 0.061 \\
  & MCD & 0.303 & 0.202  & \underline{1.030}  & 1.924 & 0.059 \\
  & DE & 0.020 & 0.156  & 1.271  & 1.806 & \underline{0.071} \\
  & HTS & 0.291 & 0.073  & 2.775  & 1.735 & 0.052 \\
  & HTS+MCD & 0.287 & 0.072  & 2.773  & \underline{1.734} & 0.050 \\
  & DUP & \underline{0.360} & \underline{0.068}  & 3.781  & 1.838 & 0.061 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{De-En}}}  
  & $\sigma^2$-fixed & -- & \underline{0.080}  & 3.053  & 1.808 & 0.018 \\
  & MCD & 0.364 & 0.210  & \underline{1.028}  & 1.908 & 0.016 \\
  & DE & 0.087 & 0.159  & 1.320  & 1.767 & \underline{0.044} \\
  & HTS & 0.326 & 0.091  & 3.015  & 1.748 & -0.002 \\
  & HTS+MCD & 0.323 & 0.091  & 3.000  & \underline{1.746} & -0.003 \\
  & DUP & \underline{0.399} & 0.081  & 3.981  & 1.837 & 0.018 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ja-En}}}  
  & $\sigma^2$-fixed & -- & 0.072  & 3.701  & 1.896 & 0.095\\
  & MCD & 0.228 & 0.229  & \underline{1.033}  & 2.082 & 0.094\\
  & DE & 0.011 & 0.143  & 1.524  & 1.845 & \underline{0.102} \\
  & HTS & 0.192 & 0.069  & 2.973  & 1.779 & 0.084 \\
  & HTS+MCD & 0.184 & 0.068  & 2.948  & \underline{1.777} & 0.082 \\
  & DUP & \underline{0.262} & \underline{0.066}  & 4.328  & 1.959 & 0.095 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Km-En}}} 
  & $\sigma^2$-fixed & -- & 0.032  & 2.613  & 1.753 & 0.208 \\
  & MCD & 0.084 & 0.145 & \underline{1.029} & 1.827 & 0.205\\
  & DE & 0.020 & \underline{0.002} & 1.207 & 2.003 & \underline{0.278} \\
  & HTS & 0.100 & 0.026  & 2.168  & 1.642 & 0.209 \\
  & HTS+MCD & 0.099 & 0.026  & 2.152  & \underline{1.640} & 0.199 \\
  & DUP & \underline{0.149} & 0.021  & 3.222  & 1.856 & 0.208 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Pl-En}}} 
  & $\sigma^2$-fixed & -- & 0.068  & 3.324  & 1.853 & 0.053 \\
  & MCD & 0.313 & 0.213 & \underline{1.031}  & 2.002 & 0.053\\
  & DE & 0.051 & 0.128  & 1.536  & 1.816 & \underline{0.065} \\
  & HTS & 0.253 & 0.069  & 2.842  & \underline{1.766} & 0.057 \\
  & HTS+MCD & 0.248 & 0.069  & 2.862  & 1.767 & 0.051 \\
  & DUP & \underline{0.358} & \underline{0.067}  & 3.922  & 1.919 & 0.053 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ps-En}}}  
  & $\sigma^2$-fixed & -- & 0.034  & 2.633  & 1.768 & 0.090 \\
  & MCD & 0.176 & 0.151 & \underline{1.029}  & 1.861 & 0.088 \\
  & DE & -0.029 & \underline{0.002}  & 1.267  & 2.134 & \underline{0.101} \\
  & HTS & 0.165 & 0.033  & 2.058  & \underline{1.647} & 0.075 \\
  & HTS+MCD & 0.159 & 0.033  & 2.044  & \underline{1.647} & 0.070 \\
  & DUP & \underline{0.218} & 0.028  & 3.267  & 1.859 & 0.090 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ru-En}}}  
  & $\sigma^2$-fixed & -- & 0.085  & 3.490  & 1.857 & 0.076 \\
  & MCD & 0.261 & 0.228 & \underline{1.030}  & 1.986 & 0.076 \\
  & DE & 0.027 & 0.153  & 1.482  & 1.815 & \underline{0.084} \\
  & HTS & 0.219 & 0.087  & 3.135  & 1.786 & 0.068 \\
  & HTS+MCD & 0.212 & 0.087  & 3.148  & \underline{1.785} & 0.067 \\
  & DUP & \underline{0.319} & \underline{0.081}  & 4.021  & 1.897 & 0.076 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ta-En}}}  
  & $\sigma^2$-fixed & -- & 0.041  & 2.069  & 1.658 & 0.108 \\
  & MCD & 0.238 & 0.121 & \underline{1.020}  & 1.688 & 0.106 \\
  & DE & 0.023 & 0.064  & 1.401  & 1.601 & \underline{0.132} \\
  & HTS & 0.245 & 0.046  & 1.704  & \underline{1.561} & 0.098 \\
  & HTS+MCD & 0.238 & 0.046  & 1.703  & 1.562 & 0.096 \\
  & DUP & \underline{0.273} & \underline{0.034}  & 2.959  & 1.767 & 0.108 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Zh-En}}}  
  & $\sigma^2$-fixed & -- & 0.076  & 3.542  & 1.886 & 0.080 \\
  & MCD & 0.309 & 0.231 & \underline{1.033} & 2.075 & 0.079 \\
  & DE & 0.034 & 0.138  & 1.527  & 1.817 & \underline{0.097} \\
  & HTS & 0.278 & 0.078  & 2.984 & \underline{1.790} & 0.071 \\
  & HTS+MCD & 0.270 & 0.078  & 2.984  & \underline{1.790} & 0.068\\
  & DUP & \underline{0.353} & \underline{0.075}  & 4.252  & 1.932 & 0.080 \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level DA predictions by BLEURT for Xx-En LPs. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_bleurt_xxen}
\end{table}



==> EMNLP 2022/table_losses.tex <==
\begin{table}[ht!]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
 &  & UPS $\uparrow$  & ECE $\downarrow$ & Sha. $\downarrow$ & NLL $\downarrow$ & PPS $\uparrow$\\  
\midrule
\multirow{3}{*}{\rotatebox{90}{\textsc{En-Xx}}} 
  & DUP ${\mathcal{L}^\mathrm{E}_{\mathrm{ABS}}}$  & 0.134  & 0.013 & 0.295 & 1.019& 0.633 \\ [3pt]
  & DUP ${\mathcal{L}^\mathrm{E}_{\mathrm{SQ}}}$  &	0.140 &	0.012 &	0.315 &	1.022 & 0.633\\ [3pt] 
  & DUP ${\mathcal{L}^\mathrm{E}_{\mathrm{HTS}}}$  & 0.146  & 0.014 & 0.293 & 1.021 &  0.633 \\ 
  \midrule
\multirow{3}{*}{\rotatebox{90}{\textsc{Xx-En}}}  
  & DUP ${\mathcal{L}^\mathrm{E}_{\mathrm{ABS}}}$   & 0.081 & 0.017 & 0.527 & 1.471 & 0.287 \\[3pt]
  & DUP ${\mathcal{L}^\mathrm{E}_{\mathrm{SQ}}}$  & 0.084  &	0.017 &	0.534 &	1.470 & 0.287\\ [3pt]
  & DUP ${\mathcal{L}^\mathrm{E}_{\mathrm{HTS}}}$  &	0.086  &	0.017 &	0.524 &	1.473 & 0.287\\ \midrule
\multirow{3}{*}{\rotatebox{90}{\textsc{Avg}}} 
  & DUP ${\mathcal{L}^\mathrm{E}_{\mathrm{ABS}}}$   & 0.104 & 1.265 & 0.015 & 0.414 & 0.446\\ [3pt]
  & DUP ${\mathcal{L}^\mathrm{E}_{\mathrm{SQ}}}$ &	0.108 &	1.262 &	0.014 &	0.427\\ [3pt]
  & DUP ${\mathcal{L}^\mathrm{E}_{\mathrm{HTS}}}$  &	0.112 &	1.266 &	0.015 &	0.411 & 0.446\\ 
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Comparison of different losses for the DUP method in segment-level DA prediction.}
\label{tab:da_losses}
\end{table}



% For calibration related indicators higher scores indicate lower performances. For correlation related indicators, higher scores indicate better performance. For each language pair the best values of each indicator are bold.

==> EMNLP 2022/table_mqm.tex <==
\begin{table}[ht!]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$  & ECE $\downarrow$ & Sha. $\downarrow$ & NLL $\downarrow$  & PPS $\uparrow$ \\  
\midrule
\multirow{5}{*}{\rotatebox{90}{\textsc{En-De}}} 
% & Baseline & 0.302 & - & 1.602 & 0.051 & 2.625 \\
& MCD  & \underline{0.134} & 0.069 & 1.019  & 0.577 & 0.295\\
  &  DE  & 0.104 & \underline{0.021} & 1.03 & 0.644 & \underline{0.332} \\
  & HTS & 0.094 & \underline{0.039} & 0.274  & 2.567 & 0.326  \\
  & HTS + MCD & 0.126 & \underline{0.021} & 0.356 & 1.502 & 0.291 \\
  & DUP & 0.038& 0.054 & \underline{0.241}  & 2.248 & 0.302 \\ 
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} & 0.302 & 0.018 & 2.241 & 0.054 & 0.243   \\ 
  \midrule %CZ to add
  \multirow{5}{*}{\rotatebox{90}{\textsc{Zh-En}}}  
%   & Baseline & 0.434 & - & 1.820 & 0.045 & 4.667  \\
  & MCD   & 0.115 & 0.081 & 1.321  & 0.956 & 0.441\\
  &  DE   & 0.14  & 0.025 & 1.143 & 0.911 & \underline{0.457}\\
  & HTS   & 0.082 & \underline{0.013} & 0.595 & 1.615 & 0.436\\
  & HTS + MCD  & -0.006  & \underline{0.013} & 0.637 & 1.42 & 0.433\\
  & DUP  & \underline{0.17}  & 0.05 & \underline{0.469} & 1.814 & 0.434\\ %   HTS + DEUP + Features (Trained on WMT20*0.7)
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} & 0.434 & 0.035 & 1.812 & 0.051 & 0.486  \\ 
  \midrule %CZ to add
\multirow{5}{*}{\rotatebox{90}{\textsc{En-Ru}}}  
% & Baseline  & 0.290 & - & 1.995 & 0.028 & 7.089 \\
& MCD    & 0.14  & 0.069 & 1.242 & 0.563 & 0.306\\
  &  DE   & 0.117  & 0.078 & 1.332 & 0.684 & 0.318\\
  & HTS  & 0.134  & 2.035 & \underline{0.306}  & \underline{0.021} & \underline{0.337}\\
  & HTS + MCD  & -0.042  & \underline{0.016} & 0.459 & 1.492 & 0.333\\
  & DUP  & \underline{0.139}  & 0.045 & 0.35 & 2.238 & 0.290\\ %   HTS + DEUP + Features (Trained on WMT20*0.7)
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} & 0.290 & 0.120 & 2.249 & 0.045 & 0.352  \\ 
  \midrule
\multirow{5}{*}{\rotatebox{90}{\textsc{AVG}}}  
% & Baseline & & & & & \\
& MCD   & 0.356 & \underline{0.129} & 0.722 & 0.074 & 1.215 \\
  &  DE  & \underline{0.377} & 0.123 & 0.763 & 0.042 & 1.179 \\
  & HTS & 0.289 & 0.079 & \underline{0.012} & 1.34 & 0.341  \\
  & HTS + MCD & 0.286 & -0.017 & 1.076 & \underline{0.011} & 0.41 \\ 
  & DUP & 0.272 & 0.115 & 1.489 & 0.035 & \underline{0.306} \\ 
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level MQM prediction without fine-tuning. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
% \andre{Excluding En-Ru, these results show that (1) HTS and DEUP are better than the estimates based on model variance (MCD and DE) in UPS, ECE, Sharpness, and worse in NLL. The En-Ru UPS is super-weird. Do we have an intuition about why there  are so many negatives? are those annotations reliable? we should consider excluding that LP if we don't trust the annotations. It looks like the problem still exists in the fine-tuned model (Tab 4). Also, are we able to add KL to this table as we have in Tab 4? Or it's only possible to consider KL in the fine-tuned model setting?}
\label{tab:mqm}
\end{table}


% For calibration related indicators higher scores indicate lower performances. For correlation related indicators, higher scores indicate better performance. For each language pair the best values of each indicator are bold.

==> EMNLP 2022/table_mqm_ft.tex <==
% \begin{table}[t]
% \small
% \centering
% \addtolength{\tabcolsep}{-0.5pt}
% \resizebox{7.7cm}{!}{
% \begin{tabular}{clccccc}
% \toprule
% &  & UPS $\uparrow$  & ECE $\downarrow$ & Sha. $\downarrow$ & NLL $\downarrow$ & PPS $\uparrow$ \\ 
% \midrule
% \multirow{6}{*}{\rotatebox{90}{\textsc{En-De}}} 
% %& Baseline & 0.374 & - & 1.796 & 0.046 & 4.780\\ 
% & MCD & 0.185 & 0.085 & 0.952 & \underline{0.631} & 0.358\\
%   &  DE  & 0.116 & \underline{0.019} & 1.034 & 0.671 & \underline{0.402}\\
%   & HTS   & \underline{0.303} & 0.029 & 0.200 & 2.001 & 0.342 \\
%   & HTS+MCD & 0.301 & 0.027 & 0.296 & 1.564 & 0.334 \\ 
%   & KL  & 0.239 & 0.049 & \underline{0.188} & 2.500 & 0.358  \\
%   & DUP   & 0.255 & 0.045 & 0.20 & 2.373 & 0.374 \\
%   \midrule 
% \multirow{6}{*}{\rotatebox{90}{\textsc{Zh-En}}}  
% %& Baseline & 0.616 & - & 1.404 & 0.016 & 1.596 \\ 
% & MCD   & 0.237 & 0.944 & 0.101 & 1.032 & 0.618 \\
%   &  DE  & 0.239 & 0.025 & 0.894 & \underline{0.869} & \underline{0.628} \\
%   & HTS  & 0.340 & 0.038 & \underline{0.487} & 1.445 & 0.599  \\
%   & HTS+MCD  & \underline{0.357} & 0.037 & 0.544 & 1.314 & 0.603 \\ 
%   & KL & 0.316 & 0.036 & 0.990 & 1.564 & 0.587 \\
%   & DUP  & 0.346 & \underline{0.012} & 0.492 & 1.290 &  0.616  \\%   HTS + DEUP + Features (Trained on WMT20*0.7)
%   %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  &  &  &  &   \\ 
%   \midrule 
% \multirow{6}{*}{\rotatebox{90}{\textsc{En-Ru}}}  
% %& Baseline & 0.371 & - & 1.624 & 0.042 & 2.876\\
% & MCD  & 0.213 & 0.09 & 1.11  & 0.69   & 0.364\\
%   &  DE   & 0.281  & 0.06 & 1.087 & \underline{0.363} & \underline{0.376}\\
%   & HTS & 0.302 & 0.075 & \underline{0.15} & 2.564  &  0.336  \\
%   & HTS+MCD & \underline{0.349} & 0.051 & 0.355  & 1.622 & 0.357 \\ 
%   & KL & 0.275 & \underline{0.044} & \underline{0.15} & 4.046 & 0.353 \\
%   & DUP   & 0.331  & 0.046 & 0.206 & 2.477 & 0.371 \\
%   \midrule
% \multirow{6}{*}{\rotatebox{90}{\textsc{Avg}}}  
% %& Baseline & & & & & \\
% & MCD    & 0.215  & 0.093 & 1.038 & 0.775 & 0.463\\
%   &  DE   & 0.222 & 0.036 & 0.997 & \underline{0.643} & \underline{0.482}\\
%   & HTS  &	0.317 &	0.048 &	\underline{0.296} &	1.976 &  0.441  \\
%   & HTS+MCD  &	\underline{0.34} &	0.039 &	0.414 &	1.485 & 0.448\\ 
%   & KL & 0.282 & 0.042 & 0.492 & 2.664 & 0.447 \\
%   & DUP   & 0.317 & \underline{0.032} & 0.317 & 1.981 & 0.469\\ %   HTS + DEUP + Features (Trained on WMT20*0.7)
%   %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  &  &  &  &  \\
% \bottomrule
% \end{tabular}
% }
% \addtolength{\tabcolsep}{-0.5pt}
% \caption{Results for segment-level MQM predictions. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
% \label{tab:mqm_ft}
% \end{table}


\begin{table}[t]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$   & ECE $\downarrow$ & Sha. $\downarrow$ & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{7}{*}{\rotatebox{90}{\textsc{En-De}}} 
& $\sigma^2$-fixed & — & 0.053  & 0.228  & 2.543 & 0.342 \\ 
& MCD & 0.132 & \underline{0.026} & 0.228 & 1.984 & 0.391 \\
& DE & 0.075 & 0.057 & \underline{0.155} & 2.911 & \underline{0.422} \\
  & HTS  & 0.236  & 0.029  & 0.192  & 2.274  & 0.370  \\
& HTS+MCD  & 0.232  & \underline{0.025}  & 0.280  & \underline{1.841}  & 0.365  \\
& KL  & \underline{0.251}  & 0.052  & \underline{0.168}  & 2.641  & 0.391  \\
& DUP  & 0.186  & 0.051  & 0.273  & 2.215  & 0.342  \\
  %   HTS + DEUP + Features (Trained on WMT20*0.7)
  %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &   \\ 
  \midrule 
\multirow{7}{*}{\rotatebox{90}{\textsc{Zh-En}}}  
& $\sigma^2$-fixed & — & 0.058  & 0.516  & 1.611 & 0.439 \\
  & MCD & 0.253 & \underline{0.009} & 0.500 & \underline{1.219} & 0.590 \\
& DE & 0.157 & 0.045 & \underline{0.420} & 1.381 & \underline{0.601} \\
  & HTS  & 0.365  & 0.036  & 0.514  & 1.338  & 0.564  \\
& HTS+MCD  & 0.380  & 0.035  & 0.566  & 1.248  & 0.570  \\
& KL  & 0.348  & 0.037  & 0.515  & 1.353  & 0.547  \\
& DUP  & \underline{0.386}  & 0.039  & 0.949  & 1.419  & 0.439  \\%   HTS + DEUP + Features (Trained on WMT20*0.7)
  %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  &  &  &  &   \\ 
  \midrule 
\multirow{7}{*}{\rotatebox{90}{\textsc{En-Ru}}}  
& $\sigma^2$-fixed & — & 0.053  & 0.338  & 2.217 & 0.340 \\
& MCD & 0.136 & 0.039 & 0.243 & 1.944 & 0.376 \\
& DE & 0.144 & 0.052 & \underline{0.100} & 3.803 & \underline{0.392} \\
 & HTS  & \underline{0.308}  & 0.059  & \underline{0.104}  & 3.317  & 0.377  \\
& HTS+MCD  & 0.304  & 0.049  & 0.285  & 1.822  & 0.375  \\
& KL  & 0.279  & 0.050  & 0.095  & 3.976  & 0.372  \\
& DUP  & 0.260  & \underline{0.029}  & 0.608  & \underline{1.783}  & 0.340  \\
%   HTS + DEUP + Features (Trained on WMT20*0.7)
  %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  &  &  &  &  \\ 
  \midrule
\multirow{7}{*}{\rotatebox{90}{\textsc{Avg}}}  
& $\sigma^2$-fixed & — & 0.055  & 0.371  & 2.090 & 0.377 \\
& MCD & 0.179 & \underline{0.024} & 0.334 & 1.686 & 0.460 \\
& DE & 0.128 & 0.051 & \underline{0.236} & 2.631 & \underline{0.479} \\
& HTS  & 0.307  & 0.041  & 0.284  & 2.264  & 0.445  \\
& HTS+MCD  & \underline{0.311}  & 0.037  & 0.388  & \underline{1.614}  & 0.445  \\
& KL  & 0.296  & 0.046  & 0.273  & 2.595  & 0.443  \\
& DUP  & 0.285  & 0.039  & 0.634  & 1.778  & 0.377  \\ %   HTS + DEUP + Features (Trained on WMT20*0.7)
  %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level MQM predictions with fine-tuning on MQM 2020 data. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:mqm_ft}
\end{table}


==> EMNLP 2022/table_param_share_dup.tex <==
\begin{table}[ht!]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
 & & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$ & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{3}{*}{\rotatebox{90}{\textsc{En-Xx}}} 
  & NS & 0.272 & 0.008  & 0.344  & 0.919 & 0.566\\ 
  & S & \underline{0.285} &	\underline{0.007} &	\underline{0.320} &	\underline{0.910} &	0.566\\ 
  & SF & 0.276 & 0.008 & 0.341 & 0.917 & 0.566  \\ 
  \midrule
\multirow{3}{*}{\rotatebox{90}{\textsc{Xx-En}}}  
  & NS &  0.090 & 0.021  & 0.546  & 1.455 & 0.334\\
  & S & 0.089 &	0.021 &	\underline{0.542} &	\underline{1.442} &	0.334\\ 
  & SF & \underline{0.093} & \underline{0.020} & 0.550 & 1.462 & 0.334 \\ \midrule
\multirow{3}{*}{\rotatebox{90}{\textsc{Avg}}} 
  & NS & 0.177 & 0.015  & 0.450  & 1.201 & 0.444\\
  & S & \underline{0.182} &	\underline{0.014} & \underline{0.437} &	\underline{1.190} &	0.444\\
  & SF & 0.180 & 0.015 & 0.451 & 1.204 & 0.444 \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Comparison of different parameter share configurations for DUP.}
\label{tab:da_param}
\end{table}


==> EMNLP 2022/table_unite_full.tex <==
% \begin{table}[!h]
% \small
% \centering
% \addtolength{\tabcolsep}{-0.5pt}
% \resizebox{6cm}{!}{
% \begin{tabular}{clccccc}
% \toprule
% &  & UPS $\uparrow$ & ECE $\uparrow$ & Sha. $\downarrow$   & NLL $\downarrow$ & PPS $\downarrow$ \\  
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Cs}}}
%   & MCD & -0.007 & 0.010  & 0.242  & 0.803 & 0.672 \\
%   & HTS & 0.151 & 0.009  & 0.427  & 0.961 & 0.718 \\
%   & HTS+MCD & 0.132 & 0.003  & 0.249  & 0.743 & 0.672 \\
%   & DUP & 0.108 & 0.011  & 0.300  & 0.988 & 0.735 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-De}}}  & MCD & 0.036 & 0.017  & 0.227  & 0.890 & 0.579 \\
%   & HTS & 0.262 & 0.030  & 0.281  & 1.064 & 0.603 \\
%   & HTS+MCD & 0.283 & 0.008  & 0.236  & 0.798 & 0.578 \\
%   & DUP & 0.241 & 0.031  & 0.207  & 1.213 & 0.623 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Ja}}}  & MCD & -0.015 & 0.008  & 0.241  & 0.775 & 0.650 \\
%   & HTS & 0.117 & 0.008  & 0.196  & 0.705 & 0.687 \\
%   & HTS+MCD & 0.148 & 0.004  & 0.229  & 0.684 & 0.646 \\
%   & DUP & 0.089 & 0.008  & 0.178  & 0.728 & 0.688 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Pl}}}  & MCD & -0.091 & 0.011  & 0.299  & 0.935 & 0.605 \\
%   & HTS & 0.127 & 0.014  & 0.481  & 1.086 & 0.626 \\
%   & HTS+MCD & 0.141 & 0.004  & 0.345  & 0.907 & 0.591 \\
%   & DUP & 0.060 & 0.013  & 0.364  & 1.133 & 0.647 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Ru}}}  & MCD & -0.059 & 0.015  & 0.248  & 0.865 & 0.587 \\
%   & HTS & 0.129 & 0.013  & 0.357  & 1.056 & 0.600 \\
%  & HTS+MCD & 0.148 & 0.009  & 0.273  & 0.890 & 0.576 \\
%  & DUP & 0.085 & 0.022  & 0.256  & 1.040 & 0.610 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Ta}}} & MCD & 0.079 & 0.005  & 0.396  & 1.052 & 0.647 \\
%  & HTS & 0.228 & 0.015  & 0.390  & 1.096 & 0.678 \\
%  & DUP & 0.164 & 0.009  & 0.371  & 1.110 & 0.685 \\
%  & HTS+MCD & 0.207 & 0.003  & 0.410  & 1.032 & 0.634 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Zh}}} & MCD & 0.177 & 0.011  & 0.214  & 0.760 & 0.504 \\
%   & HTS & 0.272 & 0.009  & 0.134  & 0.494 & 0.522 \\
%   & HTS+MCD & 0.204 & 0.002  & 0.213  & 0.622 & 0.453 \\
%  & DUP & 0.234 & 0.014  & 0.125  & 0.508 & 0.571 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Cs-En}}}  & MCD & 0.021 & 0.008  & 0.531  & 1.296 & 0.157 \\
%   & HTS & 0.049 & 0.029  & 0.474  & 1.462 & 0.171 \\
%   & HTS+MCD & 0.037 & 0.005  & 0.563  & 1.273 & 0.150 \\
%   & DUP & 0.032 & 0.027  & 0.510  & 1.490 & 0.176 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{De-En}}}   & MCD & 0.109 & 0.018  & 0.337  & 1.242 & 0.532 \\
%   & HTS & 0.116 & 0.028  & 0.390  & 1.443 & 0.554 \\
%  & HTS+MCD & 0.117 & 0.008  & 0.434  & 1.247 & 0.526 \\
%  & DUP & 0.093 & 0.036  & 0.303  & 1.532 & 0.551 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Ja-En}}}   & MCD & 0.111 & 0.005  & 0.647  & 1.289 & 0.288 \\
%  & HTS & 0.128 & 0.018  & 0.547  & 1.425 & 0.310 \\
%  & HTS+MCD & 0.116 & 0.008  & 0.669  & 1.281 & 0.280 \\
%  & DUP & 0.100 & 0.014  & 0.547  & 1.420 & 0.315 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Km-En}}}  & MCD & 0.087 & 0.015  & 0.773  & 1.272 & 0.407 \\
%  & HTS & 0.125 & 0.003  & 0.659  & 1.257 & 0.416 \\
%   & HTS+MCD & 0.124 & 0.016  & 0.944  & 1.311 & 0.396 \\
%   & DUP & 0.096 & 0.005  & 0.816  & 1.282 & 0.428 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Pl-En}}} & MCD & 0.011 & 0.022  & 0.484  & 1.408 & 0.178 \\
%  & HTS & 0.061 & 0.034  & 0.545  & 1.552 & 0.199 \\
%  & HTS+MCD & 0.053 & 0.012  & 0.523  & 1.409 & 0.181 \\
%  & DUP & 0.039 & 0.032  & 0.545  & 1.612 & 0.196 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Ps-En}}}  & MCD & 0.064 & 0.011  & 0.861  & 1.333 & 0.245 \\
%  & HTS & 0.080 & 0.005  & 0.772  & 1.353 & 0.259 \\
%  & HTS+MCD & 0.062 & 0.012  & 0.970  & 1.364 & 0.243 \\
%  & DUP & 0.068 & 0.003  & 0.803  & 1.349 & 0.260 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Ru-En}}}  & MCD & 0.048 & 0.023  & 0.411  & 1.392 & 0.210 \\
%  & HTS & 0.102 & 0.040  & 0.404  & 1.649 & 0.225 \\
%  & HTS+MCD & 0.088 & 0.011  & 0.455  & 1.351 & 0.209 \\
%   & DUP & 0.056 & 0.040  & 0.395  & 1.700 & 0.223 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Ta-En}}}  & MCD & 0.038 & 0.022  & 0.609  & 1.351 & 0.302 \\
%   & HTS & 0.073 & 0.026  & 0.648  & 1.568 & 0.320 \\
%  & HTS+MCD & 0.065 & 0.010  & 0.627  & 1.357 & 0.298 \\
%  & DUP & 0.061 & 0.030  & 0.599  & 1.592 & 0.322 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Zh-En}}}  & MCD & 0.062 & 0.017  & 0.455  & 1.417 & 0.242 \\
%  & HTS & 0.089 & 0.027  & 0.504  & 1.556 & 0.257 \\
%   & HTS+MCD & 0.071 & 0.011  & 0.480  & 1.420 & 0.238 \\
%  & DUP & 0.064 & 0.025  & 0.480  & 1.603 & 0.258 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{En-Xx}}}   & MCD & 0.022 & 0.011  & 0.260  & 0.853 & 0.603 \\
%  & HTS & 0.183 & 0.013  & 0.319  & 0.892 & 0.630 \\
%   & HTS+MCD & 0.175 & 0.004  & 0.272  & 0.792 & 0.587 \\
%   & DUP & 0.139 & 0.015  & 0.250  & 0.924 & 0.650 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{Xx-En}}}   & MCD & 0.059 & 0.016  & 0.523  & 1.352 & 0.271 \\
%  & HTS & 0.090 & 0.026  & 0.525  & 1.506 & 0.288 \\
%  & HTS+MCD & 0.079 & 0.010  & 0.572  & 1.351 & 0.267 \\
%  & DUP & 0.065 & 0.026  & 0.518  & 1.546 & 0.289 \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\textsc{AVG}}}  & MCD & 0.041 & 0.014  & 0.398  & 1.115 & 0.428 \\
% & HTS & 0.134 & 0.020  & 0.427  & 1.215 & 0.450 \\
%  & HTS+MCD & 0.124 & 0.007  & 0.429  & 1.085 & 0.419 \\
%  & DUP & 0.100 & 0.021  & 0.391  & 1.251 & 0.460 \\
% \bottomrule
% \end{tabular}
% }
% \addtolength{\tabcolsep}{-0.5pt}
% \caption{Results for segment-level DA prediction for UniTE. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
% \label{tab:da_unite}
% \end{table}

% AVERAGE
\begin{table}[!h]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$   & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Xx}}}   & $\sigma^2$-fixed & -- & 0.018  & \underline{0.224}  & 0.913 & 0.650 \\
  & MCD & 0.022 & 0.011  & 0.260  & 0.853 & 0.603 \\
  & DE & 0.129 & 0.015  & 0.264  & 0.878 & 0.647 \\
  & HTS & \underline{0.183} & 0.013  & 0.319  & 0.892 & 0.630 \\
  & HTS+MCD & 0.175 & \underline{0.004}  & 0.272  & \underline{0.792} & 0.587 \\
  & DUP & 0.139 & 0.015  & 0.250  & 0.924 & \underline{0.650} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Xx-En}}}   & $\sigma^2$-fixed & -- & 0.027  & \underline{0.498}  & 1.512 & 0.289\\
  & MCD & 0.059 & 0.016  & 0.523  & 1.352 & 0.271 \\
  & DE & 0.049 & 0.028  & 0.503  & 1.488 & \underline{0.293} \\
  & HTS & \underline{0.090} & 0.026  & 0.525  & 1.506 & 0.288 \\
  & HTS+MCD & 0.079 & \underline{0.010}  & 0.572  & \underline{1.351} & 0.267 \\
  & DUP & 0.065 & 0.026  & 0.518  & 1.546 & 0.289 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{AVG}}} 
& $\sigma^2$-fixed & -- & 0.023  & \underline{0.368}  & 1.228 & 0.460 \\
  & MCD & 0.041 & 0.014  & 0.398  & 1.115 & 0.428 \\
  & DE & 0.087 & 0.022  & 0.390  & 1.198 & \underline{0.461} \\
  & HTS & \underline{0.134} & 0.020  & 0.427  & 1.215 & 0.450 \\
  & HTS+MCD & 0.124 & \underline{0.007}  & 0.429  & \underline{1.085} & 0.419 \\
  & DUP & 0.100 & 0.021  & 0.391  & 1.251 & 0.460 \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level DA predictions by UniTE [\textbf{Average across language pairs}]. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_unite_avg}
\end{table}

% En-Xx pairs
\begin{table}[!h]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$   & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Cs}}}
  & $\sigma^2$-fixed & -- & 0.013  & 0.284  & 0.990 & \underline{0.735}\\
  & MCD & -0.007 & 0.010  & \underline{0.242}  & 0.803 & 0.672 \\
  & DE & 0.108 & 0.011  & 0.348  & 0.946 & 0.732 \\
  & HTS & \underline{0.151} & 0.009  & 0.427  & 0.961 & 0.718 \\
  & HTS+MCD & 0.132 & \underline{0.003}  & 0.249  & \underline{0.743} & 0.672 \\
  & DUP & 0.108 & 0.011  & 0.300  & 0.988 & \underline{0.735} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-De}}}  
  & $\sigma^2$-fixed & -- &  0.038  & 0.145  & 1.178 & \underline{0.623} \\
  & MCD & 0.036 & 0.017  & 0.227  & 0.890 & 0.579 \\
  & DE & 0.172 & 0.032  & \underline{0.191}  & 1.096 & \underline{0.623} \\
  & HTS & 0.262 & 0.030  & 0.281  & 1.064 & 0.603 \\
  & HTS+MCD & \underline{0.283} & \underline{0.008}  & 0.236  & \underline{0.798} & 0.578 \\
  & DUP & 0.241 & 0.031  & 0.207  & 1.213 & \underline{0.623} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ja}}}  
  & $\sigma^2$-fixed & -- &  0.011  & 0.160  & 0.718 & 0.688 \\
  & MCD & -0.015 & 0.008  & 0.241  & 0.775 & 0.650 \\
  & DE & 0.112 & 0.008  & 0.181  & \underline{0.659} & \underline{0.698} \\
  & HTS & 0.117 & 0.008  & 0.196  & 0.705 & 0.687 \\
  & HTS+MCD & \underline{0.148} & \underline{0.004}  & 0.229  & 0.684 & 0.646 \\
  & DUP & 0.089 & 0.008 & \underline{0.178}  & 0.728 & 0.688 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Pl}}}  
  & $\sigma^2$-fixed & -- &  0.014  & 0.344  & 1.124 & 0.647 \\
  & MCD & -0.091 & 0.011  & \underline{0.299}  & 0.935 & 0.605 \\
  & DE & 0.121 & 0.011  & 0.426  & 1.074 & \underline{0.652} \\
  & HTS & 0.127 & 0.014  & 0.481  & 1.086 & 0.626 \\
  & HTS+MCD & \underline{0.141} & \underline{0.004}  & 0.345  & \underline{0.907} & 0.591 \\
  & DUP & 0.060 & 0.013  & 0.364  & 1.133 & 0.647 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ru}}} 
  & $\sigma^2$-fixed & -- &  0.026  & \underline{0.229}  & 1.001 & 0.610 \\
  & MCD & -0.059 & 0.015  & 0.248  & \underline{0.865} & 0.587 \\
  & DE & 0.112 & 0.020  & 0.284  & 1.017 & \underline{0.611} \\
  & HTS & 0.129 & 0.013  & 0.357  & 1.056 & 0.600 \\
  & HTS+MCD & \underline{0.148} & \underline{0.009}  & 0.273  & 0.890 & 0.576 \\
  & DUP & 0.085 & 0.022  & 0.256  & 1.040 & 0.610 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ta}}} 
  & $\sigma^2$-fixed & -- &  0.011  & \underline{0.334}  & 1.125 & 0.685\\
  & MCD & 0.079 & 0.005  & 0.396  & 1.052 & 0.647 \\
  & DE & 0.120 & 0.018  & 0.335  & 1.089 & \underline{0.688} \\
  & HTS & \underline{0.228} & 0.015  & 0.390  & 1.096 & 0.678 \\
  & HTS+MCD & 0.207 & \underline{0.003}  & 0.410  & \underline{1.032} & 0.634 \\
  & DUP & 0.164 & 0.009  & 0.371  & 1.110 & 0.685 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Zh}}} 
  & $\sigma^2$-fixed & -- &  0.019  & \underline{0.101}  & 0.505 & \underline{0.571} \\
  & MCD & 0.177 & 0.011  & 0.214  & 0.760 & 0.504 \\
  & DE & 0.162 & 0.012  & 0.109  & \underline{0.486} & 0.546 \\
  & HTS & \underline{0.272} & 0.009  & 0.134  & 0.494 & 0.522 \\
  & HTS+MCD & 0.204 & \underline{0.002}  & 0.213  & 0.622 & 0.453 \\
  & DUP & 0.234 & 0.014  & 0.125  & 0.508 & \underline{0.571} \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level DA predictions by UniTE for En-Xx LPs. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_unite_enxx}
\end{table}



% Xx-En pairs
\begin{table}[!h]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$   & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Cs-En}}}  
  & $\sigma^2$-fixed & -- & 0.027  & 0.507  & 1.485 & 0.176  \\
  & MCD & 0.021 & 0.008  & 0.531  & 1.296 & 0.157 \\
  & DE & 0.016 & 0.029  & 0.491  & 1.454 & \underline{0.179} \\
  & HTS & \underline{0.049} & 0.029  & \underline{0.474}  & 1.462 & 0.171 \\
  & HTS+MCD & 0.037 & \underline{0.005}  & 0.563  & \underline{1.273} & 0.150 \\
  & DUP & 0.032 & 0.027  & 0.510  & 1.490 & 0.176 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{De-En}}}   
  & $\sigma^2$-fixed & -- & 0.037  & \underline{0.294}  & 1.492 & 0.551  \\
  & MCD & 0.109 & 0.018  & 0.337  & \underline{1.242} & 0.532 \\
  & DE & 0.089 & 0.033  & 0.320  & 1.437 & \underline{0.558} \\
  & HTS & 0.116 & 0.028  & 0.390  & 1.443 & 0.554 \\
  & HTS+MCD & \underline{0.117} & \underline{0.008}  & 0.434  & 1.247 & 0.526 \\
  & DUP & 0.093 & \underline{0.036}  & 0.303  & 1.532 & 0.551 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ja-En}}}   
  & $\sigma^2$-fixed & -- & 0.018  & 0.518  & 1.360 & 0.315  \\
  & MCD & 0.111 & \underline{0.005}  & 0.647  & 1.289 & 0.288 \\
  & DE & 0.073 & 0.022  & \underline{0.498}  & 1.366 & \underline{0.319} \\
  & HTS & \underline{0.128} & 0.018  & 0.547  & 1.425 & 0.310 \\
  & HTS+MCD & 0.116 & 0.008  & 0.669  & \underline{1.281} & 0.280 \\
  & DUP & 0.100 & 0.014  & 0.547  & 1.420 & 0.315 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Km-En}}}  
  & $\sigma^2$-fixed & -- & 0.006  & 0.689  & \underline{1.251} & \underline{0.428}\\
  & MCD & 0.087 & 0.015  & 0.773  & 1.272 & 0.407 \\
  & DE & 0.040 & \underline{0.003}  & \underline{0.650}  &  1.253 & 0.425 \\
  & HTS & \underline{0.125} & \underline{0.003}  & 0.659  & 1.257 & 0.416 \\
  & HTS+MCD & 0.124 & 0.016  & 0.944  & 1.311 & 0.396 \\
  & DUP & 0.096 & 0.005  & 0.816  & 1.282 & \underline{0.428} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Pl-En}}} 
  & $\sigma^2$-fixed & -- &  0.033  & 0.523  & 1.587 & 0.196  \\
  & MCD & 0.011 & 0.022  & \underline{0.484}  & \underline{1.408} & 0.178 \\
  & DE & 0.048 & 0.032  & 0.551  & 1.546 & \underline{0.202} \\
  & HTS & \underline{0.061} & 0.034 & 0.545  & 1.552 & 0.199 \\
  & HTS+MCD & 0.053 & \underline{0.012}  & 0.523  & 1.409 & 0.181 \\
  & DUP & 0.039 & 0.032  & 0.545  & 1.612 & 0.196 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ps-En}}}  
  & $\sigma^2$-fixed & -- & \underline{0.003}  & 0.792  & 1.350 & 0.260  \\
  & MCD & 0.064 & 0.011  & 0.861  & \underline{1.333} & 0.245 \\
  & DE & 0.022 & 0.004  & \underline{0.768}  & 1.342 & \underline{0.264} \\
  & HTS & \underline{0.080} & 0.005  & 0.772  & 1.353 & 0.259 \\
  & HTS+MCD & 0.062 & 0.012  & 0.970  & 1.364 & 0.243 \\
  & DUP & 0.068 & \underline{0.003}  & 0.803  & 1.349 & 0.260 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ru-En}}}  
  & $\sigma^2$-fixed & -- & 0.041  & \underline{0.368}  & 1.664 & 0.223  \\
  & MCD & 0.048 & 0.023  & 0.411  & 1.392 & 0.210 \\
  & DE & 0.064 & 0.041  & 0.385  & 1.658 & \underline{0.226} \\
  & HTS & \underline{0.102} & 0.040  & 0.404  & 1.649 & 0.225 \\
  & HTS+MCD & 0.088 & \underline{0.011}  & 0.455  & \underline{1.351} & 0.209 \\
  & DUP & 0.056 & 0.040  & 0.395  & 1.700 & 0.223 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ta-En}}}  
  & $\sigma^2$-fixed & -- &  0.031  & 0.607  & 1.481 & 0.322  \\
  & MCD & 0.038 & 0.022  & 0.609  & \underline{1.351} & 0.302 \\
  & DE & 0.035 & 0.033  & 0.605  & 1.470 & \underline{0.327} \\
  & HTS & \underline{0.073} & 0.026  & 0.648  & 1.568 & 0.320 \\
  & HTS+MCD & 0.065 & \underline{0.010}  & 0.627  & 1.357 & 0.298 \\
  & DUP & 0.061 & 0.030  & \underline{0.599}  & 1.592 & 0.322 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Zh-En}}}  
  & $\sigma^2$-fixed & -- & 0.026  & 0.468  & 1.587 & 0.258  \\
  & MCD & 0.062 & 0.017  & \underline{0.455}  & \underline{1.417} & 0.242 \\
  & DE & 0.042 & 0.027  & 0.484  & 1.552 & \underline{0.262} \\
  & HTS & \underline{0.089} & 0.027  & 0.504  & 1.556 & 0.257 \\
  & HTS+MCD & 0.071 & \underline{0.011}  & 0.480  & 1.420 & 0.238 \\
  & DUP & 0.064 & 0.025  & 0.480  & 1.603 & 0.258 \\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level DA predictions by UniTE for Xx-En LPs. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_unite_xxen}
\end{table}




==> EMNLP 2022/table_wmt20.tex <==
\begin{table}[t]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$  & NLL $\downarrow$ & PPS $\uparrow$\\  
\midrule
\multirow{5}{*}{\rotatebox{90}{\textsc{En-Xx}}} 
  & MCD   & 0.128 & 0.032 & 0.673 & 0.616 & 0.601  \\
  &  DE   & 0.134 & 0.086 & 0.461 & \underline{0.522} & \underline{0.631}\\
  & HTS   & 0.172 & 0.026 & 0.377 & 0.911 & 0.617\\
  & HTS+MCD  &	\underline{0.323} &	0.017 &	0.516 &	0.994 & 0.609\\
  & DUP   & 0.285 &	\underline{0.007} &	\underline{0.320} &	0.910 &	0.566\\
  \midrule
\multirow{5}{*}{\rotatebox{90}{\textsc{Xx-En}}}  
& MCD    & 0.019 & 0.073 & 1.432 & 1.033 & 0.286\\
  &  DE  & 0.044 & 0.086 & 1.131 & \underline{0.943} & 0.296 \\
  & HTS  & 0.079 & \underline{0.011} & 0.566 & 1.441 & 0.278 \\
  & HTS+MCD &	\underline{0.176} &	\underline{0.011} &	0.600 &	1.323 & 0.276 \\
  & DUP  & 0.089 &	0.021 &	\underline{0.542} &	1.442 &	\underline{0.334}\\
  %0.086 & 0.017 & \underline{0.524} & 1.473 & 0.287 \\
  \midrule
\multirow{5}{*}{\rotatebox{90}{\textsc{Avg}}}  
& MCD   & 0.071 & 0.053 & 1.083 & 0.816 & 0.435 \\
  &  DE  & 0.090 & 0.086 & 0.813 & \underline{0.728} & \underline{0.455} \\
  & HTS  & 0.119 & 0.020 & 0.466 & 1.189 & 0.435 \\
  & HTS+MCD & \underline{0.254} & \underline{0.013} & 0.528 & 1.167  & 0.429 \\ 
  & DUP  & 0.182 &	0.014 & \underline{0.437} &	1.190 &	0.444\\
  %0.112 & 0.015 & \underline{0.411} & 1.266 & 0.446 \\ %  
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{%\ricardo{Why is the PPS in the last column here and in the first column in Table 2} 
Results for segment-level DA predictions. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_seg_notqe}
\end{table}

% \underline{Underlined} numbers indicate the best result for each language pair and evaluation metric. Reported are the predictive Pearson score $r(\hat{\mu},q^*)$ (PPS), the uncertainty Pearson score $r(|q^*-\hat{\mu}|,\hat{\sigma})$ (UPS), the negative  log-likelihood (NLL), the expected calibration error (ECE), and the sharpness (Sha.)

% For calibration related indicators higher scores indicate lower performances. For correlation related indicators, higher scores indicate better performance. For each language pair the best values of each indicator are bold.

%% ORIGINAL copy
% \begin{table}[t]
% \small
% \centering
% \addtolength{\tabcolsep}{-0.5pt}
% \resizebox{7.7cm}{!}{
% \begin{tabular}{clccccc}
% \toprule
% &  & PPS $\uparrow$ & UPS $\uparrow$ & NLL $\downarrow$   & ECE $\downarrow$ & Sha. $\downarrow$ \\  
% \midrule
% \multirow{5}{*}{\rotatebox{90}{\textsc{En-Xx}}} 
% & MCD  & 0.601 & 0.128 & 0.616 & 0.032 & 0.673   \\
%   &  DE  & 0.631 & 0.134 & \underline{0.522} & 0.086 & 0.461 \\
%   & HTS  & 0.617 & 0.172 & 0.911 & 0.026 & 0.377 \\
%   & HTS+MCD & 0.609 &	\underline{0.323} &	0.994 &	0.017 &	0.516\\
%   & DUP  & \underline{0.633} & 0.145 & 1.021 & \underline{0.013} & \underline{0.293} \\%   HTS + DEUP + Features (Trained on WMT20*0.7)
%   %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  0.633 &	0.140 &	1.016 & 0.013	&	0.296   \\ 
%   \midrule
% \multirow{5}{*}{\rotatebox{90}{\textsc{Xx-En}}}  
% & MCD   & 0.286 & 0.019 & 1.033 & 0.073 & 1.432 \\
%   &  DE  & \underline{0.296} & 0.044 & \underline{0.943} & 0.086 & 1.131 \\
%   & HTS  & 0.278 & 0.079 & 1.441 & \underline{0.011} & 0.566 \\
%   & HTS+MCD & 0.276 &	\underline{0.176} &	1.323 &	\underline{0.011} &	0.600  \\
% %   & DEUP_{L1}  & 0.286 & 0.080 & 1.474 & 0.017 & 0.521 \\ %DEUP
% %   & DEUP_{L2} & 0.286 &	0.080 & 1.474 & 0.018 &	0.521  \\ %CZ to add
% %   & DEUP_{L3} &  &  &  &  & \\ % CZ to add: HTS + DEUP
%   & DUP  & 0.287 & 0.086 & 1.473 & 0.017 & \underline{0.524} \\%   HTS + DEUP + Features (Trained on WMT20*0.7)
%   %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} & 0.287	& 0.074 &	1.470 & 0.017	& 0.531  \\ 
%   \midrule
% \multirow{5}{*}{\rotatebox{90}{\textsc{Avg}}}  
% & MCD   & 0.435 & 0.071 & 0.816 & 0.053 & 1.083 \\
%   &  DE  & \underline{0.455} & 0.090 & \underline{0.728} & 0.086 & 0.813 \\
%   & HTS  & 0.435 & 0.119 & 1.189 & 0.020 & 0.466 \\
%   & HTS+MCD & 0.429 & \underline{0.254} &	1.167 &	\underline{0.013} &	0.528 \\ 
% %   & DEUP_{L1}  & 0.446 & 0.099 & 1.275 & 0.016 & 0.408 \\ 
% %   & DEUP_{L2} &0.446 & 0.105 &	1.279 &	0.017 &	0.427 \\ 
% %   & DEUP_{L3} &  &  &  &  & \\ % CZ to add: HTS + DEUP
%   & DUP  & 0.446 & 0.112 & 1.266 & 0.015 & \underline{0.411} \\ %   HTS + DEUP + Features (Trained on WMT20*0.7)
% %  & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} & 0.446  & 0.101 & 1.233 & 0.015 & 0.417  \\  
% \bottomrule
% \end{tabular}
% }
% \addtolength{\tabcolsep}{-0.5pt}
% \caption{Results for segment-level DA predictions. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
% \label{tab:da_seg_notqe}
% \end{table}

==> EMNLP 2022/table_wmt20_enxx.tex <==
\begin{table}[!h]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$   & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Cs}}} 
& $\sigma^2$-fixed  & --    &  0.005  & 0.408  & 1.019 & 0.699 \\
& MCD  & 0.149 & 0.012  & 0.258  & 0.847 & 0.692   \\
  &  DE & 0.125 & 0.010  & \underline{0.255}  & \underline{0.825} & \underline{0.734} \\
  & HTS  & 0.105 & \underline{0.003}  & 0.456  & 1.025 & 0.699 \\
  & HTS+MCD & \underline{0.335} & 0.008 & 0.388 & 0.880 & 0.676 \\
  & DUP &  0.146 & \underline{0.003} & 0.419 & 1.010 & 0.699 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  &  &  &  &   \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-De}}}
& $\sigma^2$-fixed  & --    & 0.032  & \underline{0.172}  & 1.106 & 0.586 \\
& MCD  & 0.284 & 0.013  & 0.260  & \underline{0.916} & 0.582 \\
  &  DE & 0.209 & 0.025  & 0.198  & 0.949 & \underline{0.616} \\
  &  HTS  &  0.231 & 0.022  & 0.243  & 1.016 & 0.586 \\
  & HTS+MCD  & \underline{0.386} & \underline{0.004} & 0.369 & 0.924 & 0.612 \\ 
  & DUP & 0.232 & 0.022 & 0.190 & 1.028 & 0.586 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ja}}} 
& $\sigma^2$-fixed  & --    & 0.011  & 0.186  & 0.714 & 0.636 \\
& MCD  & 0.236 & 0.005  & 0.225  & 0.697 & 0.638 \\
  &  DE & 0.140 & 0.010  & \underline{0.179}  & \underline{0.657} & 0.661 \\
  &  HTS  & 0.184 & 0.007  & 0.218  & 0.691 & 0.636\\
  & HTS+MCD   & \underline{0.249}  & \underline{0.003} & 0.520 & 1.048 & \underline{0.669} \\
  & DUP & 0.220 & 0.005 & 0.201 & 0.679 & 0.636 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Pl}}}  
& $\sigma^2$-fixed  & --    & 0.010  & 0.410  & 1.090 & 0.609 \\
  & MCD & 0.167 & 0.010  & 0.326  & \underline{0.947} & 0.610  \\
  & DE & 0.129 & 0.011  & \underline{0.315}  & 0.960 & \underline{0.645} \\
  & HTS & 0.103 & 0.008  & 0.436  & 1.095 & 0.609 \\
  & HTS+MCD & \underline{0.189} & \underline{0.004} & 0.397 & 0.969 & 0.631\\
  & DUP  & 0.112 & 0.004 & 0.431 & 1.094 & 0.609 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ru}}}
& $\sigma^2$-fixed  & --    & 0.018  & 0.287  & 0.989 & 0.534 \\
& MCD   & 0.200 & 0.012  & 0.307  & 0.943 & 0.538 \\
  &  DE & 0.146 & 0.016  & \underline{0.263}  & \underline{0.898} & \underline{0.570} \\
  &  HTS  & 0.156 & 0.012  & 0.321  & 1.006 & 0.534 \\
  & HTS+MCD  & \underline{0.370} & 0.017 & 0.637 & 1.050 & 0.497 \\
  & DUP & 0.154 & \underline{0.009} & 0.305 & 0.991 & 0.534 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ta}}}
& $\sigma^2$-fixed  & --    &  0.017  & \underline{0.356}  & 1.077 & 0.661\\
& MCD   & 0.077 & \underline{0.004}  & 0.406  & 1.035 & 0.658  \\
  &  DE & 0.111 & 0.010  & 0.361  & \underline{1.030} & \underline{0.676} \\
  &  HTS  & 0.250 & 0.009  & 0.435  & 1.050 & 0.661\\
  & HTS+MCD  & 0.231 & 0.038 & 0.921 & 1.223 & 0.617 \\
  & DUP & \underline{0.252} & 0.009 & 0.385 & 1.032 & 0.661 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Zh}}}
& $\sigma^2$-fixed  & --    & 0.017  & 0.173  & 1.016 & 0.325 \\
& MCD  & 0.083 & 0.018  & \underline{0.152}  & 1.367 & 0.330  \\
  &  DE & 0.560 & 0.021  & \underline{0.152}  & 0.813 & 0.327 \\
  &  HTS  & 0.728 & \underline{0.003}  & 0.273  & 0.657 & 0.325 \\
  & HTS+MCD  & 0.504 & 0.020 & 0.380 & 0.865 & \underline{0.562} \\
  & DUP & \underline{0.722} & \underline{0.003} & 0.268 & \underline{0.650} & 0.325 \\ \midrule
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\ 
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Xx}}} 
& $\sigma^2$-fixed  & --    & 0.015  & 0.288  & 1.000 & 0.566 \\
  & MCD   & 0.163 & 0.011  & 0.265  & 0.984 & 0.566  \\
  &  DE  & 0.223 & 0.015  & \underline{0.240}  & \underline{0.864} & 0.591\\
  & HTS   & 0.272 & 0.008  & 0.344  & 0.919 & 0.566\\
  & HTS+MCD  &	\underline{0.323} &	0.017 &	0.516 &	0.994 & \underline{0.609}\\
  & DUP   & 0.285 &	\underline{0.007} &	0.320 &	0.910 &	0.566\\
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level DA prediction for En-Xx LPs. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_notqe_enxx}
\end{table}



==> EMNLP 2022/table_wmt20_xxen.tex <==
\begin{table}[ht!]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&   & UPS $\uparrow$   & ECE $\downarrow$ & Sha. $\downarrow$ & NLL $\downarrow$ & PPS $\uparrow$\\  
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Cs-En}}} 
& $\sigma^2$-fixed  & --    &  0.026  & 0.509  & 1.422 & 0.216 \\
& MCD  & 0.099 & 0.012  & 0.462  & 1.319 & 0.215  \\
  &  DE & 0.134 & 0.019  & \underline{0.366}  & 1.156 & \underline{0.460} \\
  & HTS  & 0.077 & 0.024  & 0.518  & 1.432 & 0.216 \\
  & HTS+MCD   & \underline{0.229} & \underline{0.006} & 0.502 & \underline{1.276} & 0.195\\
  & DUP & 0.082 & 0.024 & 0.516 & 1.418 & 0.216 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  &  &  &  &   \\ 
  \midrule 
\multirow{6}{*}{\rotatebox{90}{\textsc{De-En}}} 
& $\sigma^2$-fixed  & --    & 0.025  & 0.403  & 1.398 & 0.573  \\
& MCD   & 0.044 & 0.030  & \underline{0.312}  & 1.343 & 0.568 \\
  &  DE & 0.056 & 0.030  & 0.321  & 1.374 & \underline{0.574} \\
  &  HTS  & 0.099 & 0.024  & 0.425  & 1.389 & 0.573 \\
  & HTS+MCD  & \underline{0.148} & \underline{0.014} & 0.463 & \underline{1.107} & 0.563 \\
  & DUP  & 0.100 & 0.023 & 0.432 & 1.382 & 0.573\\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\ 
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ja-En}}}
& $\sigma^2$-fixed  & --    &  0.020  & 0.494  & 1.344 & 0.348 \\
& MCD  & 0.064 & 0.008  & 0.532  & \underline{1.280} & 0.349 \\
  &  DE & 0.079 & 0.012  & \underline{0.502}  & 1.305 & \underline{0.360} \\
  &  HTS  & 0.145 & 0.015  & 0.534  & 1.351 & 0.348 \\
  & HTS+MCD & \underline{0.215} & \underline{0.007} & 0.611 & 1.322 & 0.339 \\
  & DUP & 0.129 & 0.016 & 0.513 & 1.333 & 0.348 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\ 
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Km-En}}} 
& $\sigma^2$-fixed  & --    &  0.007  & 0.618  & 1.246 & 0.452 \\
& MCD  & 0.012 & 0.005  & 0.663  & 1.235 & 0.453 \\
  &  DE & 0.067 & \underline{0.003}  & \underline{0.631}  & \underline{1.226} & \underline{0.464} \\
  &  HTS  & \underline{0.147} & 0.004  & 0.661  & 1.255 & 0.452 \\
  & HTS+MCD  & 0.143 & 0.015 & 0.836 & 1.263 & 0.452  \\
  & DUP  & 0.144 & 0.004 & 0.638 & 1.239 & 0.452 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\ 
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Pl-En}}}
& $\sigma^2$-fixed  & --    &  0.027  & 0.586  & 1.518 & 0.264 \\
& MCD  & 0.063 & 0.029  & \underline{0.472}  & 1.450 & 0.265  \\
  &  DE & 0.029 & 0.029  & 0.500  & 1.490 & \underline{0.271} \\
  &  HTS  & 0.045 & 0.025  & 0.609  & 1.530 & 0.264 \\
  & HTS+MCD  & \underline{0.139} & \underline{0.008} & 0.502  & \underline{1.424} & 0.268 \\
  & DUP  & 0.048 & 0.025 & 0.604 & 1.519 & 0.264 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\ 
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ps-En}}}
& $\sigma^2$-fixed  & --    &  0.005  & 0.735  & 1.319 & 0.325 \\
& MCD & 0.028 & 0.006  & 0.740  & \underline{1.291} & 0.327 \\
  &  DE & 0.040 & \underline{0.004}  & \underline{0.732}  & 1.295 & \underline{0.330} \\
  &  HTS  & 0.110 & 0.005  & 0.735  & 1.315 & 0.325 \\
  & HTS+MCD & \underline{0.111} & 0.013 & 0.849 & 1.315 & 0.297 \\
  & DUP  & 0.097 & 0.005 & \underline{0.732} & 1.317 & 0.325 \\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\ 
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ru-En}}}
& $\sigma^2$-fixed  & --    & 0.031  & 0.454  & 1.574 & 0.288  \\
& MCD & 0.058 & 0.033  & \underline{0.373}  & 1.528 & 0.281  \\
  &  DE & 0.056 & 0.034  & 0.401  & 1.526 & \underline{0.300} \\
  &  HTS  & 0.087 & 0.030  & 0.464  & 1.575 & 0.288 \\
  & HTS+MCD  & \underline{0.161} & \underline{0.013} & 0.493 & \underline{1.520} & 0.209\\
  & DUP  & 0.073 & 0.029 & 0.467 & 1.570 & 0.288\\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\ 
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Ta-En}}}
& $\sigma^2$-fixed  & --    &  0.028  & 0.588  & 1.416 & 0.346 \\
& MCD  & 0.047 & 0.022  & \underline{0.567}  & 1.357 & 0.346 \\
  &  DE & 0.058 & 0.024  & 0.585  & 1.410 & \underline{0.357} \\
  &  HTS  & 0.081 & 0.023  & 0.577  & 1.468 & 0.346 \\
  & HTS+MCD   & \underline{0.250} & \underline{0.016} & 0.642 & \underline{1.300} & 0.284\\
  & DUP  & 0.079 & 0.025 & 0.602 & 1.420 & 0.346\\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\ 
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Zh-En}}}
& $\sigma^2$-fixed  & --    &  0.021  & 0.518  & 1.510 & 0.303 \\
& MCD  & 0.051 & 0.020  & \underline{0.447}  & 1.458 & 0.302 \\
  &  DE &  0.054 & 0.022  & 0.451  & 1.481 & \underline{0.310} \\
  &  HTS  & 0.082 & 0.020  & 0.533  & 1.508 & 0.303 \\
  & HTS+MCD  & \underline{0.186} & \underline{0.006} & 0.504 & \underline{1.377} & 0.278 \\
  & DUP  & 0.089 & 0.020 & 0.523 & 1.502 & 0.303 \\\midrule
  \multirow{6}{*}{\rotatebox{90}{\textsc{Xx-En}}} 
  & $\sigma^2$-fixed  & --    & 0.023  & 0.529  & 1.448 & 0.334 \\
& MCD    & 0.055 & 0.020  & \underline{0.477}  & 1.392 & 0.332\\
  &  DE  & 0.053 & 0.022  & 0.480  & 1.418 & \underline{0.342} \\
  & HTS  & 0.090 & 0.021  & 0.546  & 1.455 & 0.334 \\
  & HTS+MCD &	\underline{0.176} &	\underline{0.011} &	0.600 &	\underline{1.323} & 0.276 \\
  & DUP  & 0.089 &	0.021 &	0.542 &	1.442 &	0.334\\
%   & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3}  &  &  &  &  & \\ 
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level DA prediction for Xx-En LPs. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_notqe_xxen}
\end{table}


==> EMNLP 2022/ted_full.tex <==
\begin{table}[t]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$   & ECE $\downarrow$ & Sha. $\downarrow$ & NLL $\downarrow$ & PPS $\uparrow$ \\  
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-De}}}  
& $\sigma^2$-fixed  & --    & 0.072 & \underline{0.146} & 2.957 & 0.526 \\
& MCD     & 0.178 & \underline{0.052} & 0.147 & 2.500 & 0.540 \\
& DE      & 0.371 & 0.062 & 0.314 & 1.977 & \underline{0.571} \\
& HTS     & 0.290 & 0.070 & 0.251 & 2.239 & 0.425 \\
& HTS+MCD & \underline{0.401} & 0.073 & 0.227 & \underline{1.756} & 0.545 \\
& DE      & 0.346 & 0.058 & 0.346 & 2.219 & 0.526\\\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{En-Ru}}}  
& $\sigma^2$-fixed  & --    & 0.057 & 0.229 & 2.095 & 0.436 \\
& MCD     & 0.086 & 0.065 & 0.238 & 1.846 & 0.425 \\
& DE      & 0.271 & 0.057 & 0.346 & 1.679 & \underline{0.441} \\
& HTS     & 0.267 & 0.084 & \underline{0.151} & 2.506 & 0.372 \\
& HTS+MCD & \underline{0.293} & 0.068 & 0.402 & \underline{1.473} & 0.387 \\
& DUP     & 0.282 & \underline{0.047} & 0.300 & 1.781 & 0.436 \\\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Zh-En}}}  
& $\sigma^2$-fixed  & --    & 0.033 & 0.397 & 2.203 & 0.434 \\
& MCD     & 0.063 & \underline{0.023} & 0.283 & 2.348 & 0.447 \\
& DE      & 0.23  & 0.036 & 0.586 & 1.865 & 0.456 \\
& HTS     & \underline{0.378} & 0.067 & \underline{0.135} & 2.685 & \underline{0.544} \\
& HTS+MCD & 0.288 & 0.073 & 0.223 & 2.276 & 0.425 \\
& DUP     & 0.271 & 0.030 & 0.825 & \underline{1.718} & 0.434\\ \bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Results for segment-level MQM predictions on TEDTalk data. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:ted_full}
\end{table}

==> table_wmt20.tex <==
\begin{table}[t]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
\resizebox{7.7cm}{!}{
\begin{tabular}{clccccc}
\toprule
&  & UPS $\uparrow$ & ECE $\downarrow$ & Sha. $\downarrow$  & NLL $\downarrow$ & PPS $\uparrow$\\  
\midrule
\multirow{5}{*}{\rotatebox{90}{\textsc{En-Xx}}} 
  & MCD   & 0.128 & 0.032 & 0.673 & 0.616 & 0.601  \\
  &  DE   & 0.134 & 0.086 & 0.461 & \underline{0.522} & \underline{0.631}\\
  & HTS   & 0.172 & 0.026 & 0.377 & 0.911 & 0.617\\
  & HTS+MCD  &	\underline{0.323} &	0.017 &	0.516 &	0.994 & 0.609\\
  & DUP   & 0.285 &	\underline{0.007} &	\underline{0.320} &	0.910 &	0.566\\
  \midrule
\multirow{5}{*}{\rotatebox{90}{\textsc{Xx-En}}}  
& MCD    & 0.019 & 0.073 & 1.432 & 1.033 & 0.286\\
  &  DE  & 0.044 & 0.086 & 1.131 & \underline{0.943} & 0.296 \\
  & HTS  & 0.079 & \underline{0.011} & 0.566 & 1.441 & 0.278 \\
  & HTS+MCD &	\underline{0.176} &	\underline{0.011} &	0.600 &	1.323 & 0.276 \\
  & DUP  & 0.089 &	0.021 &	\underline{0.542} &	1.442 &	\underline{0.334}\\
  %0.086 & 0.017 & \underline{0.524} & 1.473 & 0.287 \\
  \midrule
\multirow{5}{*}{\rotatebox{90}{\textsc{Avg}}}  
& MCD   & 0.071 & 0.053 & 1.083 & 0.816 & 0.435 \\
  &  DE  & 0.090 & 0.086 & 0.813 & \underline{0.728} & \underline{0.455} \\
  & HTS  & 0.119 & 0.020 & 0.466 & 1.189 & 0.435 \\
  & HTS+MCD & \underline{0.254} & \underline{0.013} & 0.528 & 1.167  & 0.429 \\ 
  & DUP  & 0.182 &	0.014 & \underline{0.437} &	1.190 &	0.444\\
  %0.112 & 0.015 & \underline{0.411} & 1.266 & 0.446 \\ %  
\bottomrule
\end{tabular}
}
\addtolength{\tabcolsep}{-0.5pt}
\caption{%\ricardo{Why is the PPS in the last column here and in the first column in Table 2} 
Results for segment-level DA predictions. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
\label{tab:da_seg_notqe}
\end{table}

% \underline{Underlined} numbers indicate the best result for each language pair and evaluation metric. Reported are the predictive Pearson score $r(\hat{\mu},q^*)$ (PPS), the uncertainty Pearson score $r(|q^*-\hat{\mu}|,\hat{\sigma})$ (UPS), the negative  log-likelihood (NLL), the expected calibration error (ECE), and the sharpness (Sha.)

% For calibration related indicators higher scores indicate lower performances. For correlation related indicators, higher scores indicate better performance. For each language pair the best values of each indicator are bold.

%% ORIGINAL copy
% \begin{table}[t]
% \small
% \centering
% \addtolength{\tabcolsep}{-0.5pt}
% \resizebox{7.7cm}{!}{
% \begin{tabular}{clccccc}
% \toprule
% &  & PPS $\uparrow$ & UPS $\uparrow$ & NLL $\downarrow$   & ECE $\downarrow$ & Sha. $\downarrow$ \\  
% \midrule
% \multirow{5}{*}{\rotatebox{90}{\textsc{En-Xx}}} 
% & MCD  & 0.601 & 0.128 & 0.616 & 0.032 & 0.673   \\
%   &  DE  & 0.631 & 0.134 & \underline{0.522} & 0.086 & 0.461 \\
%   & HTS  & 0.617 & 0.172 & 0.911 & 0.026 & 0.377 \\
%   & HTS+MCD & 0.609 &	\underline{0.323} &	0.994 &	0.017 &	0.516\\
%   & DUP  & \underline{0.633} & 0.145 & 1.021 & \underline{0.013} & \underline{0.293} \\%   HTS + DEUP + Features (Trained on WMT20*0.7)
%   %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} &  0.633 &	0.140 &	1.016 & 0.013	&	0.296   \\ 
%   \midrule
% \multirow{5}{*}{\rotatebox{90}{\textsc{Xx-En}}}  
% & MCD   & 0.286 & 0.019 & 1.033 & 0.073 & 1.432 \\
%   &  DE  & \underline{0.296} & 0.044 & \underline{0.943} & 0.086 & 1.131 \\
%   & HTS  & 0.278 & 0.079 & 1.441 & \underline{0.011} & 0.566 \\
%   & HTS+MCD & 0.276 &	\underline{0.176} &	1.323 &	\underline{0.011} &	0.600  \\
% %   & DEUP_{L1}  & 0.286 & 0.080 & 1.474 & 0.017 & 0.521 \\ %DEUP
% %   & DEUP_{L2} & 0.286 &	0.080 & 1.474 & 0.018 &	0.521  \\ %CZ to add
% %   & DEUP_{L3} &  &  &  &  & \\ % CZ to add: HTS + DEUP
%   & DUP  & 0.287 & 0.086 & 1.473 & 0.017 & \underline{0.524} \\%   HTS + DEUP + Features (Trained on WMT20*0.7)
%   %& DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} & 0.287	& 0.074 &	1.470 & 0.017	& 0.531  \\ 
%   \midrule
% \multirow{5}{*}{\rotatebox{90}{\textsc{Avg}}}  
% & MCD   & 0.435 & 0.071 & 0.816 & 0.053 & 1.083 \\
%   &  DE  & \underline{0.455} & 0.090 & \underline{0.728} & 0.086 & 0.813 \\
%   & HTS  & 0.435 & 0.119 & 1.189 & 0.020 & 0.466 \\
%   & HTS+MCD & 0.429 & \underline{0.254} &	1.167 &	\underline{0.013} &	0.528 \\ 
% %   & DEUP_{L1}  & 0.446 & 0.099 & 1.275 & 0.016 & 0.408 \\ 
% %   & DEUP_{L2} &0.446 & 0.105 &	1.279 &	0.017 &	0.427 \\ 
% %   & DEUP_{L3} &  &  &  &  & \\ % CZ to add: HTS + DEUP
%   & DUP  & 0.446 & 0.112 & 1.266 & 0.015 & \underline{0.411} \\ %   HTS + DEUP + Features (Trained on WMT20*0.7)
% %  & DUP_{f_\mathrm{\{Q,MCD\}}}^{L_3} & 0.446  & 0.101 & 1.233 & 0.015 & 0.417  \\  
% \bottomrule
% \end{tabular}
% }
% \addtolength{\tabcolsep}{-0.5pt}
% \caption{Results for segment-level DA predictions. \underline{Underlined} numbers indicate the best result for each evaluation metric in each language pair.}
% \label{tab:da_seg_notqe}
% \end{table}
